A Graph to Graphs Framework for Retrosynthesis Prediction

A fundamental problem in computational chemistry is to find a set of reactants to synthesize a target molecule, a.k.a. retrosynthesis prediction. Existing state-of-the-art methods rely on matching the target molecule with a large set of reaction templates, which are very computationally expensive and also suffer from the problem of coverage. In this paper, we propose a novel template-free approach called G2Gs by transforming a target molecular graph into a set of reactant molecular graphs. G2Gs first splits the target molecular graph into a set of synthons by identifying the reaction centers, and then translates the synthons to the final reactant graphs via a variational graph translation framework. Experimental results show that G2Gs significantly outperforms existing template-free approaches by up to 63% in terms of the top-1 accuracy and achieves a performance close to that of state-of-the-art template based approaches, but does not require domain knowledge and is much more scalable.

==> Retrosynthesis Camera Ready/0-abstract.tex <==
\begin{abstract}
\iffalse
We tackle a fundamental problem in computational chemistry known as retrosynthesis prediction, which aims to identify reactants that can produce a specified product.
The problem is challenging since it is an abductive reasoning process and the computation cost of searching the transformation space is expensive.
%Retrosynthesis prediction is a fundamental problem in computational chemistry.
The current state-of-the-art approaches rely on template-based models to select reaction rules, which suffer from coverage and scalability issues. In this work, we formulate the task as a graph-to-graph translation problem and
propose \textit{Variational Graph Translation Network (\modelname)}, a novel template-free 
generative model for retrosynthesis prediction.
%\modelname~ predicts reactants by first identifying reaction centers on product graphs, and then predicting the leaving groups for each synthon split from product graphs according to reaction centers.
%\modelname enjoys xxxxx
%Given a target product, 
\modelname~first splits the product into synthons by identifying reaction centers, and then 
%generates reactants based on synthons using a novel encoder-decoder graph translation architecture.
generates reactants via a series of graph transformations from synthons.
Experiment results show that \modelname~achieves competitive performance compared with state-of-the-art template-based baselines, with up to 63\% improvement in terms of the top-1 accuracy compared with the template-free baseline.
\fi 

A fundamental problem in computational chemistry is to find a set of reactants to synthesize a target molecule, a.k.a. retrosynthesis prediction. Existing state-of-the-art methods rely on matching the target molecule with a large set of reaction templates, which are very computationally expensive and also suffer from the problem of coverage. In this paper, we propose a novel template-free approach called \modelname by transforming a target molecular graph into a set of reactant molecular graphs. \modelname first splits the target molecular graph into a set of synthons by identifying the reaction centers, and then translates the synthons to the final reactant graphs via a variational graph translation framework. Experimental results show that \modelname significantly outperforms existing template-free approaches by up to 63\%  %improvement 
in terms of the top-1 accuracy 
%and is close to the performance of 
and achieves a performance  close to that of 
state-of-the-art template-based approaches, 
but does not require domain knowledge and is much more scalable.
The code is available at \url{https://github.com/DeepGraphLearning/torchdrug}. 


\iffalse
Retrosynthesis prediction, which devotes to  find a set of reactants to synthesize a target molecule, is a fundamental process in computational chemistry. 
Despite their great potentials for  synthesis planning, state-of-the-art  computational methods rely on matching the target molecule with a large set of reaction templates. Such approaches, however, not only require expensive computation but also suffer from poor generalization on  new target structures and reaction types. To address these limitations, we propose a   template-free strategy, \modelname, which aims to effectively transform a target molecular graph into a set of reactant molecular graphs.  In a nutshell, \modelname first splits the target molecular graph into a set of synthons, which are then translated  into the final reactant graphs through  a variational graph translation  network. 
We experimentally show that \modelname  outperforms existing template-free approaches by up to 63\%  in terms of  top-1 accuracy. These numbers are also matching that obtained by the state-of-the-art template-based strategies, but our method excludes the need for  domain knowledge and  scales well  to larger data sets, making it  particularly attractive in practice.
\fi
\end{abstract}

==> Retrosynthesis Camera Ready/1-introduction.tex <==
\section{Introduction}
%brief introduction to the problem. the significance/challenge of the problem.
Retrosynthesis, which devotes to find a set of reactants to synthesize a target molecule, is of crucial importance to the synthesis planning and drug discovery. The problem is challenging as the search space of all possible transformations is huge by nature. For decades, people have been seeking to aid retrosynthesis analysis with modern computer techniques~\citep{retro1969computer_aid}. Among them, machine learning plays a vital role and significant progress has been made recently~\citep{sara2016computer_retro, connor2018ml_retro}.

%% template based (pros and cons)
Existing machine learning works on retrosynthesis prediction mainly fall into two categories: template-based~\cite{Connor2017retrosim, Marwin2017neuralsym, Dai2019GLN} and template-free models~\cite{liu2017retro_seq2seq, pavel2019retro_transformer}. 
The template-based approaches  
%Most existing  works on retrosynthesis prediction rely on
match the target molecule with a large set of reaction templates, which define the subgraph patterns of a set of chemical reactions. For example,~\citep{Connor2017retrosim} proposed a similarity-based approach to select reaction templates for the target molecule.~\citep{Marwin2017neuralsym, Javier2019retro_multiscale_class} cast rule selection as a multi-class classification problem. Recently,~\citep{Dai2019GLN} treats chemistry knowledge as logic rules and directly models the joint probability of rules and reactants, which achieves the new state of the art.
Despite their great potential for synthesis planning, template-based methods, however, not only require expensive computation but also suffer from poor generalization on new target structures and reaction types.
%Inspired by the recent advances in neural machine translation ~\citep{bahdanau2014nmt, vaswani2017transformer}, another line of research for retrosynthesis prediction~\citep{liu2017retro_seq2seq, pavel2019retro_transformer} bypasses reaction templates and formulates retrosynthesis prediction as a sequence-to-sequence problem on SMILES~\citep{weininger1988smiles} representation of molecules.
Another line of research for retrosynthesis  prediction~\citep{liu2017retro_seq2seq, pavel2019retro_transformer} bypasses reaction templates and formulates retrosynthesis prediction as a sequence-to-sequence problem. Such approaches leverage the 
 recent advances in neural machine translation ~\citep{bahdanau2014nmt, vaswani2017transformer} and the  SMILES~\citep{weininger1988smiles} representation of molecules.
However, SMILES representation assumes a sequential order between the atoms in a molecule, which cannot effectively reflect the complex relationships between atoms in a molecule. 
%capture molecule similarity~\citep{jin2018junction}, and  assumes a sequential order for a molecule, whose structure is non-euclidean. %Therefore, these approaches are apt to ignore rich chemical context of molecular graphs, and the performance has been unsatisfactory so far. 
As a result, these approaches fail to capture the rich chemical contexts and their interplays of molecules, resulting in  unsatisfactory  predictive performance. 




\iffalse
%% template free is underexplored.
Recently, there has been significant advances in neural machine translation with various sequence-to-sequence models, e.g., recurrent neural networks~\citep{bahdanau2014nmt} and transformer~\citep{vaswani2017transformer}. Inspired by this,~\citep{liu2017retro_seq2seq, pavel2019retro_transformer} bypass reaction templates and formulate retrosynthesis prediction as a sequence-to-sequence problem on SMILES representation of molecules. However, SMILES representation is not designed to capture molecule similarity~\citep{jin2018junction} , and it assumes a sequential order for a molecule, whose structure is non-euclidean. Therefore, these approaches are apt to ignore rich chemical context of molecular graphs, and the performance has been unsatisfactory so far. 
\fi

To address the aforementioned issues, 
%In this paper,
in this paper we represent each molecule as a graph and formulate retrosynthesis prediction as a graph-to-graphs translation problem. The so-called G2Gs leverages the powerful representation of graph for molecule and is a novel template-free approach, which is trained with an extensive collection of molecule reaction data.
%, and devise a novel template-free approach. % called G2Gs. 
%G2Gs, built upon deep neural networks, consists of two key components: (1) a reaction center identification module that reduce the one-to-many graph translation problem into the one-to-one graph translation problem, by splitting synthons from the target molecule; (2) a variational graph translation module that translates a synthon to a final reactant graph. 
%The so-called G2Gs method leverages the representation power and training efficiency of deep graphic models. 
Specifically, it consists of two key components: (1) a reaction center identification module, which splits synthons from the target molecule and reduces the one-to-many graph translation problem into multiple one-to-one  translation processes; (2) a variational graph translation module, which translates a synthon to a final reactant graph. 
%In the first step, to effectively predict the reaction center, we use graph neural networks~\cite{duvenaud2015convolutional,kearnes2016molecular,gilmer2017neural} to encode both the local structure (\textit{i.e.}, the edges) and the global structure (\textit{i.e.}, the entire graph) for the prediction. 
We aim to model the probability of reactant graph $G$ conditioned on the synthon $S$, \textit{i.e.}, $P(G|S)$. As a synthon could be potentially translated to different reactants in different reaction contexts, a latent code $z$ is introduced to handle the uncertainty of reactant prediction, \textit{i.e.}, $P(G|z,S)$. Following existing work on graph generation~\cite{you2018graph, liu2018constrained, shi*2020graphaf}, we formulate reactant graph generation as a sequential decision process, more specifically, sequentially generating nodes and edges. The whole graph translation process can be efficiently and effectively optimized with the variational inference approach~\citep{kingma2014vae}. 

%As a result, G2Gs attains the advantages of both template-based and template-free models. 
%As a template-free method, \modelname does not require any domain knowledge, and is able to generate 100\% chemically valid predictions by incorporating validity check during the graph translation. Also, the whole framework can be efficiently trained as it bypasses reaction templates and subgraph isomorphism.
%Promisingly, its translation procedure serves as the reverse process of a chemical reaction, which offers great interpretability and insight for synthesis planning.

We evaluate our model on the benchmark data set USPTO-50k derived from a patent database~\citep{daniel2012phdthesis}, and compare it with both template-based and template-free approaches.
%\footnote{Code and data are available at \href{Anonymous}{Anonymous}}.
We experimentally show that \modelname significantly outperforms existing template-free baselines by up to 63\% in terms of the top-1 accuracy. These numbers are also approaching those obtained by the state-of-the-art template-based strategies, but our method excludes the need for domain knowledge and scales well to larger data sets, making it particularly attractive in practice.
%and is able to generate 100\% chemically valid predictions by incorporating validity check during the graph translation. Meanwhile

%\textcolor{blue}{
\iffalse
Our main contributions can be summarized as follows.
\begin{itemize}
%\item We propose a novel graph to graphs framework called G2Gs for retrosynthesis prediction. G2Gs is a template-free based approach and include two different stages: reaction center prediction and synthon to reactant graph translation.
\item We novelly formulate retrosynthesis prediction as a graph-to-graphs translation process and propose \modelname for the challenging task.
%\item We propose to leverage both the local and global structure information in molecules for reaction center prediction, and a variational graph translation approach to translate the synthon to the final reactant graph, which effectively handles the uncertainty of the translation process.
\item We devise a variational translation method to address the uncertainty and diversity in graph translation.  
%\item Experimental results show that G2Gs achieve the state-of-the-art performance compared to existing template-free approaches and is close to the state-of-the-art template-based approach, but much more efficient and scalable.
\item We experimentally verify the superior performance of our proposed graph translation paradigm for retrosynthesis prediction.  
\end{itemize}
%}
\fi

\iffalse
Retrosynthesis prediction, which devotes to  find a set of reactants to synthesize a target molecule, is a fundamental process in computational chemistry. 
Despite their great potentials for  synthesis planning, state-of-the-art  computational methods rely on matching the target molecule with a large set of reaction templates. Such approaches, however, not only require expensive computation but also suffer from poor generalization on  new target structures and reaction types. To address these limitations, we propose a   template-free strategy, \modelname, which aims to effectively transform a target molecular graph into a set of reactant molecular graphs.  In a nutshell, \modelname first splits the target molecular graph into a set of synthons, which are then translated  into the final reactant graphs through  a variational graph translation  network. 
We experimentally show that \modelname  outperforms existing template-free approaches by up to 63\%  in terms of  top-1 accuracy. These numbers are also matching that obtained by the state-of-the-art template-based strategies, but our method excludes the need for  domain knowledge and  scales well  to larger data sets, making it  particularly attractive in practice.
\fi

==> Retrosynthesis Camera Ready/2-related_work.tex <==
%\section{Background}
%In this section, we first briefly introduce the concept of chemical reaction and retrosynthesis prediction, and then review three lines of research related to our work.

%\subsection{Chemical Reaction and Retrosynthesis}

\section{Related Work}

\textbf{Retrosynthesis Prediction }
%\paragraph{Template-based Approach}
Prior works on retrosynthesis prediction are primarily based on reaction templates, which are either hand-crafted by human experts~\citep{Markus2011reaction_template, sara2016computer_retro} or extracted from large chemical databases automatically~\citep{connor2017pred_react}.
Since there are hundreds of qualified templates for a target molecule by subgraph matching, selecting templates that lead to chemically feasible reactions remains a crucial challenge for these approaches.
To cope with such challenge,  \citep{Connor2017retrosim} proposed to select templates based on similar reactions in the data set.~\citep{Marwin2017neuralsym, Javier2019retro_multiscale_class} further employed neural models for rule selection. The state-of-the-art method~\citep{Dai2019GLN} %is built upon graph neural networks, where 
leveraged the idea that 
the templates and reactants are hierarchically sampled from their conditional joint distributions. Such template-based approaches, however, still  suffer from poor generalization on unseen structures and reaction types, and the computational cost for subgraph isomorphism in these methods is often prohibitively expensive.

%\paragraph{Template-free Approach}
To overcome the limitation of template-based methods, template-free approaches have recently been actively investigated.    ~\citep{liu2017retro_seq2seq, pavel2019retro_transformer} formulated the task as a sequence-to-sequence problem on SMILES representation of molecules, and the same idea was adopted in~\citep{philippe2017transformer, Schwaller2018MolecularTF} for its dual problem, \textit{i.e.}, organic reaction prediction. However, these approaches are apt to ignore the rich chemical contexts  contained in the graph structures of molecules, and the validity of the generated SMILES strings can not be ensured, resulting in unsatisfactory performance. %, as one edit on a SMILES string can lead to a totally invalid molecule. 
In contrast, our \modelname framework, directly operating on the graph structures of molecules, is able to generate 100\% chemically valid predictions with high accuracy, while excludes the need for  reaction templates and computationally expensive graph isomorphism.

%\textcolor{blue}{
Our work is also related to the chemical reaction prediction method presented in~\citep{jin2017weisfeiler} in terms of learning a neural model for reaction center identification. Nevertheless, both the  definition of the reaction center and the targeted task, namely  retrosynthesis prediction, 
distinguish our strategy from their algorithm. 

%}


\textbf{Molecular Graph Generation }
Various deep generative models for molecular graph generation have recently been introduced~\cite{segler2017generating,olivecrona2017molecular,samanta2018designing,neil2018exploring,you2018graph, liu2018constrained, shi*2020graphaf}. %Among them, 
Our \modelname framework is closely related to the state-of-the-art models that decompose the generation process into a sequence of graph transformation steps, including~\cite{you2018graph, liu2018constrained, shi*2020graphaf}. In these approaches, the generation procedure is formulated as a sequential decision making process by dynamically adding new nodes and edges based on current subgraph structures. For example,  \cite{you2018graph} introduced a reinforce policy network for the decision making.  \cite{shi*2020graphaf} presented an alternative sequential generation algorithm based on autoregressive flow called GraphAF. \cite{liu2018constrained} combined sequential generation with a variational autoencoder to enable continuous graph optimization in the latent space.
%In the retrosynthesis scenario, given specified product molecule, the reactants could be slightly different with diverse reaction conditions such as reagent and temperature. To mitigate this underlying multi-modality problem, in \modelname we also explicitly introduce low-dimensional latent variables to modulate the sequential graph translation process, which helps us to model the diverse output distributions.

Unlike the aforementioned approaches, we here leverage  graph generation for retrosynthesis prediction, where novel components have to be devised for this specific task. For example, in the retrosynthesis scenario, given a specified product molecule, the reactants could be slightly different with diverse reaction conditions such as reagent and temperature. To cope with such intrinsic  multi-modality problem, in \modelname we also explicitly introduce low-dimensional latent variables to modulate the sequential graph translation process, aiming at  capturing the diverse output distributions.


==> Retrosynthesis Camera Ready/3-model.tex <==
% \newpage
\begin{figure}[tbhp]
	\centering
    \includegraphics[width=.79\linewidth]{figure/Fig1_v3-crop.pdf}
    \caption{The overall framework of the proposed method. The reaction center identified by \modelname is marked in red. The product graph  is first split into synthons by disconnecting the reaction center. Based on resulted synthons, reactants are then generated via a series of graph transformations. The generated molecule scaffolds are bounded by blue bounding box.}
    \label{fig:framework}
    \vspace{-7pt}
\end{figure}

\section{The Graph to Graphs Framework}\label{sec:model}

%overall introduction
%two phase, pipeline
%In this paper, we formulate the retrosynthesis task as a one-to-many graph-to-graphs translation problem and propose to tackle the problem in a two-step fashion. Given the specified product molecular graph, \modelname first splits the product graph into synthons by identifying reaction centers via graph representation learning approach, and then translates the synthons to the final reactants using a novel variational graph translation module. More specifically, we first employ a graph neural network to estimate the reactivity score of all atom pairs of the product graph, and the atom pair with the highest reactivity score above a threshold will be selected as the reaction center. After the reaction center is pinpointed, we split the product graph into synthons by disconnecting the bond of reaction center. Then, starting from the synthons, the reactants are generated via a series of graph transformations. With different reaction conditions such as reagent and temperature, the mapping from a synthon to a reactant may not be unique, therefore we also incorporate a latent vector to encourage the model to capture the uncertainty and generate diverse predictions. The overall framework is illustrated in Figure~\ref{fig:framework}. In this section, we first formally introduce the notations and notions used throughout the paper, and then elaborate the details of modules in our proposed G2Gs framework.
%introduce key concepts including notation, chemical reaction & retrosynthesis.
In this paper, we formulate the retrosynthesis task as a one-to-many graph-to-graphs translation problem. % and propose to tackle the problem in a two-step fashion.
%Given the specified product molecular graph, \modelname first splits the product graph into synthons by identifying reaction centers via graph representation learning approach, and then translates the synthons to the final reactants using a novel variational graph translation module. More specifically, 
In specific, we first employ a graph neural network to estimate the reactivity score of all atom pairs of the product graph, and the atom pair with the highest reactivity score above a threshold will be selected as the reaction center. We then split the product graph into synthons by disconnecting the bonds of the reaction center resulted. Finally, basing on the obtained synthons, the reactants are generated via a series of graph transformations, where a latent vector is employed to encourage the model to capture the transformation uncertainty and generate diverse predictions.
%With different reaction conditions such as reagent and temperature, the mapping from a synthon to a reactant may not be unique, therefore we also incorporate a latent vector to encourage the model to capture the uncertainty and generate diverse predictions. 
The proposed framework is illustrated in Figure~\ref{fig:framework}, and will be  discussed in  detail next. % In this section, we first formally introduce the notations and notions used throughout the paper, and then elaborate the details of modules in our proposed G2Gs framework.
%introduce key concepts including notation, chemical reaction & retrosynthesis.

\subsection{Preliminaries}
\label{subsec:nation_notation}

\textbf{Notation }
In this paper, a molecule is represented as a labeled graph $G = (A, X)$, where $A$ is the adjacency matrix and $X$ the matrix of node features. Let the number of atoms be $n$, the number of bond types be $b$, and the dimension of node features be $d$, then we have $A \in \{0, 1\}^{n \times n \times b}$ and $X \in \{0, 1\}^{n \times d}$. $A_{ijk}=1$ here indicates a bond with type $k$ between the $i^{th}$ and $j^{th}$ nodes.

\textbf{Retrosynthesis Prediction }
Formally, a chemical reaction can be represented as a pair of two sets of molecules $(\{G_i\}_{i=1}^{N_1}, \{G_j\}_{j=1}^{N_2})$, where $G_i$ denotes a reactant graph and $G_j$  a product graph. In retrosynthesis prediction, given the set of products $\{G_j\}_{j=1}^{N_2}$, the goal is to precisely predict the set of reactants $\{G_i\}_{i=1}^{N_1}$. Following existing work, in this paper we focus on the standard single-outcome reaction case, \textit{i.e.}, $N_2=1$, and thus simplifying  the  notation of a reaction $r$ as $(\{G_i\}_{i=1}^{N_1}, G_p)$. 

\textbf{Reaction Center and Synthon }\label{reaction_center}
Unlike that in~\citep{jin2017weisfeiler},  the phrase \textit{reaction center} here is used to represent an atom pair $(i, j)$ that satisfies two conditions: (1) there is a bond between the  $i^{th}$ and $j^{th}$ nodes in the product graph; (2) there is no  bond between the  $i^{th}$ and $j^{th}$ nodes in the reactant graph. 
% Note that all the reactions are \textit{atom-mapped} and each atom in the reactant set has a unique index.
Also, synthons are subgraphs extracted from the products by breaking the bonds in the reaction centers. These synthons can later be transformed into reactants, %\textcolor{red}{That being said}, a synthon is a subgraph within the product, which can be transformed into a reactant.
and a synthon may not be a valid molecule.

%\subsection{Molecular Graph Representation Learning}
\textbf{Molecular Graph Representation Learning }
\label{subsec:rgcn}
Graph Convolutional Networks (GCN)~\citep{duvenaud2015convolutional,kearnes2016molecular,kipf2016semi,gilmer2017neural,schutt2017quantum} have achieved great success in representation learning for computational chemistry. Given a molecular graph $G=(A, X)$, we adopt a variant of Relational GCN (R-GCN)~\citep{schlichtkrull2018modeling} to compute both the node embeddings and the graph-level embedding. Let $k$ $\in \mathbb{R}$ be the embedding dimension and $H^l \in \mathbb{R}^{n\times k}$  the node embeddings at the $l^{th}$ layer computed by the R-GCN $(H^0 = X)$. $H^l_i$ represents the embedding of the $i^{th}$ atom. At each layer, the R-GCN calculates the embedding for each node by aggregating messages from  different edge types:
\begin{equation}
%\begin{aligned}
%&\tilde{E}_{i}=A_{[:,:,i]} + I
H^{l}=\operatorname{Agg}\left(\operatorname{ReLU}\big(\{E_{i} H^{l-1} W_{i}^{l}\} \big| i \in(1, \ldots, b)\big)\right)
%\end{aligned}
\end{equation}
where $E_{i} = A_{[:,:,i]} + I$ denotes the adjacency matrix of the $i^{th}$ edge type with self-loop and $ W_{i}^{l}$ is the trainable weight matrix for the $i^{th}$ edge type. $\operatorname{Agg}(\cdot)$ denotes an aggregation function chosen from summation, averaging and concatenation. 
We stack $L$ R-GCN layers to compute the final node embeddings $H^L$. The entire graph-level embedding $h_G$ can also be calculated by applying a $\operatorname{Readout}(\cdot)$ function to $H^L$~\cite{hamilton2017inductive}, \textit{e.g.}, summation.
%Assume we stack $L$ R-GCN layers,
%the whole graph embeddings $h$ can be calculated by applying a readout function to the node embeddings computed at $L^{th}$ layer:


\subsection{Reaction Center Identification}\label{subsec:reaction_center}
Given a chemical reaction $(\{G_i\}_{i=1}^{N_1}, G_p)$, we first derive a binary label matrix $Y \in \{0, 1\}^{n \times n}$ for each atom pair (\textit{i.e.}, bond) in the product $G_p$, indicating the reaction centers as defined in Section~\ref{subsec:nation_notation}; $Y_{ij}=1$ here indicates that the bond between $i^{th}$ and $j^{th}$ node in $G_p$ is a reaction center. It is worth noting that, both the reactants and the product are \textit{atom-indexed}. That is, each atom in the reactant set is associated with a unique index. This property enables us to  identify the reaction centers by simply comparing each pair of atoms in the product $G_p$ with that in a reactant $G_i$, forming the binary label matrix $Y$. With such label matrix, the Reaction Center Identification procedure in G2Gs is then formulated as a binary link prediction task as follows.


We use a $L$-layer R-GCN defined in Section~\ref{subsec:rgcn} to compute the node embeddings $H^L$ and the entire graph embedding $h_{G_p}$ of product $G_p$:
\begin{equation}
H^{L} = \operatorname{R-GCN} (G_p), \  h_{G_p}= \operatorname{Readout} (H^{L}).
\end{equation}
To estimate the reactivity score of the atom pair $(i, j)$, the edge embedding $e_{ij}$ is formed by concatenating  the node embeddings of the $i^{th}$ and $j^{th}$ nodes as well as the one-hot bond type feature. In addition, since a $L$-layer R-GCN can only gather information within $L$ hops of the center node, but the reactivity of a reaction center may also be affected by the remote atoms, we also enable the edge embedding  $e_{ij}$ to take into account the graph embedding (\textit{i.e.}, global structure), so as to leverage the knowledge of the remote atoms. 
Formally, we have:
\begin{equation}
e_{ij} = H^L_i \ \Vert \ H^L_j \  \Vert \ A_{ij} \ \Vert \ h_{G_p}
\end{equation}
where $\Vert$ denotes the vector concatenation operation. $H_i^L \in \mathbb{R}^k$ denotes the $i^{th}$ row of $H^L$ and $A_{ij}=A_{[i,j,:]} \in \{0, 1\}^b$ is the edge type of the atom pair $(i, j)$ in $G_p$. 
%\textcolor{red}{Note that the reaction class can also be incorporated in the edge embedding if available.}
The final reactivity score of the atom pair $(i,j)$ is calculated as:
\begin{equation}
s_{ij} = \sigma(m_r(e_{ij}))
\end{equation}
where $m_r$ is a feedforward network that maps $e_{ij}$ to a scalar, and $\sigma(\cdot)$ denotes the $\operatorname{Sigmoid}$ function. In the case that a certain reaction type is known during retrosynthesis analysis, we can also include this information by concatenating its embedding to the input of the feedforward network, \textit{i.e.}, $e_{ij}$.

%\textbf{Learning }
For learning, the reaction center identification module can be optimized by maximizing the cross entropy of the binary label matrix $Y$ as follows:
\begin{equation}
    \mathcal{L}_1 = -\sum\limits_{r}\sum\limits_{i \neq j  } \lambda Y_{ij}\text{log}(s_{ij}) +  (1-Y_{ij})\text{log}(1-s_{ij})
\end{equation}
where $\lambda \in [1, + \infty)$ is a weighting hyper-parameter, with the following purpose. In practice, among all the atom pairs there are typically a few reaction centers. As a result, the output logit of the feedforward network $m_r$ is often extremely small. Through  the weighting  $\lambda$, we are able to  alleviate such issue caused by the imbalanced class distributions.

%\textbf{Inference }
During  inference, we first calculate the reactivity scores of all atom pairs, and then select the highest one above a threshold as the reaction center. %, \textit{i.e.}, if all the scores are below the threshold, then no reaction center is identified. One alternative way is to enumerate 
Alternatively, one can select 
the top-$k$ atom pairs with the highest  scores above a threshold as the reaction center. This scenario will  yield more diverse synthesis routes but with the cost of inference time.
% Currently we assume that a reaction has at most one reaction center, which accounts for 98\% of the dataset. 

%After the reaction center is pinpointed, we then disconnect the bond of the reaction center in $G_p$, and treat each connected subgraph in $G_p$ as a synthon. Note that, in the case that none of the reaction center is identified, the product $G_p$ itself will be considered as a synthon. Once we extract synthons from the product $G_p$, the G2Gs problem is turned into one-to-one graph translations, \textit{i.e.}, translating each synthon to the final reactant graph.
After collecting reaction centers, we then disconnect the bonds of the reaction centers in $G_p$, and treat each connected subgraph in $G_p$ as a synthon. Note that, in the case that none of the reaction center is identified, the product $G_p$ itself will be considered as a synthon. Doing so, we can extract all the synthons from the product $G_p$, and then formulate a one-to-one graph translation procedure to translate each resulted synthon to a final reactant graph. We will discuss this translation process in detail next. 

\begin{figure*}[hbtp]
	\centering
    \includegraphics[width=.80\linewidth]{figure/Fig2_v2-crop.pdf}
    \caption{Illustration of the proposed variational graph translation module, including the encoder $q(z|G,S)$ (left) and the generative model $p(G|z,S)$ (right). The phases of the generation procedure are shown in the generative model. With a sampled latent vector $z$, the synthon graph $S$ enters a loop with nodes selection and edge labeling until the termination state is predicted.}
    %The looped arrow to $S^i$ indicates that several iterations of the illustrated steps may happen to generate a final target reactant graph $G$.}
    \label{fig:syn2graph}
    \vspace{-7pt}
\end{figure*}

\subsection{Reactants Generation via Variational Graph Translation}
%In this section, we elaborate the procedure that how synthons are translated into the final reactant graphs through our proposed variational graph translation module.
Given a chemical reaction $(\{G_i\}_{i=1}^{N_1}, G_p)$, we denote the set of synthons extracted from $G_p$ (as discussed in Section~\ref{subsec:reaction_center}) as $\{S_i\}_{i=1}^{N_1}$. For simplicity, we omit the subscript and denote a translation pair as $(S, G)$. %In this module we aim to learn a conditional generative model $p(G|S)$ that recover the reactant molecule domain ($G$) from the synthon molecule domain ($S$). In this scenario, a common problem is that the same synthon can be translated to different reactants which is known as the multi-modal problem.
In this setting, our goal  is to  learn a conditional generative model $p(G|S)$ that recovers the reactant molecule domain ($G$) from the synthon molecule domain ($S$). 
It is worth noting that, an intrinsic issue is that the same synthon can be translated to different reactants, which is known as the multi-modality problem.
% Note that $\mathcal{F}$ is a many-to-many mapping, i.e., a synthon can be translated to different reactants while a reactant can also be translated from different synthons. 
In order to mitigate such multi-modality problem and encourage the module to model the diverse distribution of reactants, we incorporate a low-dimensional latent vector $z$ to capture the uncertainty for the graph translation process. Details are discussed next. 
%, and adopt an encoder-decoder architecture for the graph translation.


\subsubsection{The Generative Model}\label{subsubsec:generative_model}
We build upon previous works on graph generation models~\cite{li2018learning,you2018graphrnn}. 
%We define the translation of a synthon $S$ to the final reactant $G$ as a conditional generative procedure $p(G|S)$. As mentioned above, we introduce latent variables and formulate this graph translation in a variational autoencoder framework to solve the multi-model problem. In this section, we concentrate on the generation (\textit{a.k.a.} decoding) procedure, where $G$ is generated conditioned on the $S$ and a latent vector $z$.
The generation of graph $G$ is conditioned on both the $S$ and the latent vector $z$.
% \textcolor{red}{add the reason that we choose to model this distribution insted of $p(G| z, S)$}
%In practice, we first autoregressively generate a sequence of graph transformation actions $(a_1, \cdots, a_T)$, and then applying them on the initial synthon graph $S$. Here $a_t$ is a one-step graph transformation (action) acts as a modification of the graph. Thus, we turn the problem of modeling $p(G|z,S)$ to the joint distribution over the sequence of graph transformation actions $p(a_{1:T} | z, S)$. With such a generative model, a synthon can be translated into a reactant by sampling action sequences from the distribution. Next, we describe the details of the generative procedure.
In detail, we first autoregressively generate a sequence of graph transformation actions $(a_1, \cdots, a_T)$, and then apply them on the initial synthon graph $S$. Here $a_t$ is a one-step graph transformation (\textit{i.e.}, action) acting as a modification to the graph. Formally, let $\mathcal{T}$ be the collection of all trajectories $(a_1, \cdots, a_T)$ that can translate synthons $S$ to target reactants $G$ and $t \in \mathcal{T}$ be a possible trace. Then, we factorize  modeling $p(G|z,S)$ into modeling the joint distribution over the sequence of graph transformation actions $p(t | z, S)$. The connection between $p(G|z,S)$ and $p(t | z, S)$ is illustrated in Section~\ref{subsubsec:step2-learning}. With such a generative model, a synthon can be translated into a reactant by sampling action sequences from the distribution. Next, we describe the details of the generative procedure.

Let $S^{i}$ denote the graph after applying the sequence of actions $a_{1:i}$ to $S$, and $S^0 = S$. Then we have $p(S^i|S^{i-1},z)=p(a_{i}|S^{i-1},z)$. In previous graph generation models~\cite{li2018learning,you2018graphrnn}, each decision $a_i$ is conditioned on a full history of the generation sequence ($S^0, \cdots, S^{i-1}$), which leads to the stability and scalability problems arising from the optimization process. 
%\textcolor{red}{
To alleviate these issues, 
our graph translation dynamics leverages the assumption of a Markov Decision Process (MDP), which satisfies
% \textcolor{red}{How so? be more specific here? heuristic or proof?}
the Markov property that $p(S^i|S^{i-1},z)=p(S^i|S^{i-1},\cdots,S^0,z)$. The MDP formulation means that each action is only conditioned on the graph that has been modified so far. Hence the graph translation model $p(t | z, S)$ can be naturally factorized as follows:
\begin{equation}\label{eq:trace_fact}
p(t|z,S) = p(a_{1:T} | z, S) =
\prod\limits_{i=1}^T p(a_{i} | z, S^{i-1}).
\end{equation}

Before we detail the parameterization of distribution $P(a_{i} | z, S^{i-1})$, we formally introduce the definition of an action. An action $a_i$ is a tuple with four elements:
\begin{equation}
a_i = (a_{i}^1, a_{i}^2, a_{i}^3, a_{i}^4).
\end{equation}
Assuming the number of atom types is $m$, then $a_{i}^1 \in \{0, 1\}^2$ predicts the termination of the  graph translation procedure; $a_{i}^2 \in \{0, 1\}^n$ indicates the first node to focus; $a_{i}^3 \in \{0, 1\}^{n+m}$ indicates the second node to focus; $a_{i}^4 \in \{0, 1\}^b$ predicts the type of bond between two nodes. Then the distribution $p(a_{i} | z, S^{i-1})$ can be further decomposed into three parts: (1) termination prediction $p(a_{i}^1 | z, S^{i-1})$; (2) nodes selection $p(a_{i}^{2:3}, | z, S^{i-1}, a_{i}^1) $; (3) edge labeling $p(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3})$.
We will discuss the parameterization of these components in detail next. %in the following paragraphs.

\textbf{Termination Prediction }
Denote a $L$-layer R-GCN (Section~\ref{subsec:rgcn}) that can compute the node embeddings of an input graph as $\mathcal{R}(\cdot)$.
We parameterize the distribution as:
\begin{equation}\label{eq:term_pred}
\begin{aligned}
&H = \mathcal{R}(S^{i-1}), \  h_{S}= \operatorname{Readout} (H)  \\
&p(a_{i}^1 | z, S^{i-1}) = 
\tau\big(m_t(h_{S}, z)\big)
\end{aligned}
\end{equation}
where $\tau(\cdot)$ denotes the softmax function, and $m_t(\cdot)$ is a feedforward network. At each transformation step, we sample $a_{i}^1 \sim p(a_{i}^1 | z, S^{i-1})$. If $a_{i}^1$ indicates the termination, then the graph translation process will stop, and the  current graph $S^{i-1}$ is treated as the final reactant $G$ generated by the module. 


\textbf{Nodes Selection }
Let the set of possible atoms (\textit{e.g.}, carbon, oxygen) to be added during graph translation be $\{v_1, \cdots, v_m\}$ and denote the collection as $V= \bigcup_{i=1}^m v_i$.
We first extend the graph $S^{i-1}$ to $\tilde{S}^{i-1}$ by adding isolated atoms, \textit{i.e.}, $\tilde{S}^{i-1} = S^{i-1} \bigcup V$.
The first node is selected from atoms in $S^{i-1}$, while the second node is selected from $\tilde{S}^{i-1}$ conditioned on the first node, by concatenating its embeddings with embeddings of each atom in $\tilde{S}^{i-1}$:
\begin{equation}\label{eq:node_select}
\begin{aligned}
&p(a_{i}^2 | z, S^{i-1}, a_{i}^1) = \tau
\big(
\beta_1 \odot
m_f(\mathcal{R}(\tilde{S}^{i-1}), z)
\big)\\
&a_{i}^2 \sim p(a_{i}^2 | z, S^{i-1}, a_{i}^1)\\
&p(a_{i}^3 | z, S^{i-1}, a_{i}^{1:2}) = \tau
\big(
\beta_2 \odot
m_s(\mathcal{R}(\tilde{S}^{i-1}), z, a_{i}^2)
\big)\\
&a_{i}^3 \sim p(a_{i}^3 | z, S^{i-1}, a_{i}^{1:2})\\
\end{aligned}
\end{equation}
where $m_f(\cdot)$ and $m_s(\cdot)$ are feedforward networks. $\beta_1$ and $\beta_2$ are masks to zero out the probability of certain atoms being selected. 
Specifically, $\beta_1$ forces the module to select node from $S^{i-1}$, and $\beta_2$ prevents the first node from being selected again.
In this case, only the second node can be selected from $V$, and it corresponds to adding a new atom to $S^{i-1}$.
The distribution of node selection $p(a_{i}^{2:3}, | z, S^{i-1}, a_{i}^1)$ is the product of the two conditional distributions  described above.


\textbf{Edge Labeling }
The distribution for edge labeling is parameterized as follows:
\begin{equation}\label{eq:edge_label}
\begin{aligned}
&p(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3}) = \tau
\big(
m_e(\mathcal{R}(\tilde{S}^{i-1}), z, a_{i}^{2:3})
\big)\\
&a_{i}^4 \sim P(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3})\\
\end{aligned}
\end{equation}
where $m_e(\cdot)$ is a feedforward networks. The knowledge of reaction classes can be incorporated in the same way as in Section~\ref{subsec:reaction_center}.

%We leave  the details of the feedforward networks described above and  \textcolor{red}{other architectures in supplementary material}. \textcolor{blue}{Note that the knowledge about reaction classes can be incorporated to the input of each feedforward networks if available.}

Given these distributions,
the distribution $p(t | z, S)$ can be parameterized according to~\cref{eq:trace_fact,eq:term_pred,eq:node_select,eq:edge_label}. 
Finally, the probability of translating the synthon $S$ to the final reactant $G$ can be computed by enumerating all possible graph transformation sequences that translate $S$ to $G$: 
\begin{equation}\label{eq:logp_gzs}
P(G|z, S) = \sum\limits_{t \in \mathcal{T}}
P(t | z, S)
\end{equation}

\subsubsection{Learning}
\label{subsubsec:step2-learning}
To learn the parameters of our variational graph translation module, we aim to maximize the log likelihood of the observed translation pair, \textit{i.e.}, $logP(G|S)$. Directly optimizing the objective involves marginalizing the latent variable $z$, which is computationally intractable. To this end, we turn to the standard amortized variational inference~\citep{kingma2014vae} by introducing an approximate posterior $q(z|G, S)$, which is modeled as a Gaussian distribution to allow effectively sampling $z$ via the reparameterization trick.
%with a mean of $\mu$ and a variance of $\text{diag}(\sigma^2)$. 
In specific, the mean and the log variance of $q(z|G, S)$ are parameterized as follows:
\begin{equation}
\begin{aligned}
& \mu = m_{\mu}(h_G \Vert h_S)\\
& \text{log}\sigma^2 = m_{\sigma}(h_G \Vert h_S)\\   
& q(z|G, S) = \mathcal{N}(z \vert \mu, \text{diag}(\sigma^2)) \\
\end{aligned}
\end{equation}
where the $h_G$ and $h_S$ are graph embeddings of $G$ and $S$ respectively, computed by the same R-GCN. $m_{\mu}(\cdot)$ and  $m_{\sigma}(\cdot)$ are feedforward networks. The evidence lower bound (ELBO) is then defined as:
\begin{equation}
\mathcal{L}_{\text{ELBO}} = \mathbb{E}_{z \sim q}[\text{log}P(G|z,S)] - \operatorname{KL}[q(z|G, S) \Vert p(z|S)]
\end{equation}
where $\operatorname{KL}[q(\cdot) \Vert p(\cdot)]$ is the Kullback-Leibler divergence between $q(\cdot)$ and $p(\cdot)$. We here take the prior $p(z|S)$ as a standard Gaussian $\mathcal{N}(z | 0, I)$. 

\textbf{Efficient Training }
The computation of $\text{log}P(G|z,S)$ (eq.~\ref{eq:logp_gzs}) is expensive as it
requires the summation over all possible graph transformation sequences that translate $S$ to $G$. 
Here we introduce two strategies that perform well empirically. 
We first show that $\text{log}P(G|z,S)$ is lower bounded by the expected log likelihood of all the trajectories $t=(a_1,\cdots,a_T)$ that translate $S$ to $G$ using Jensen{'}s inequality:
\begin{equation}
\begin{aligned}
\text{log}P(G|z, S) &= \text{log}\sum\limits_{t \in \mathcal{T}}
P(t | z, S)\\
&\geq \text{log}|t| + \frac{1}{|t|}\sum\limits_{t \in \mathcal{T}}\text{log}P(t | z, S)
\end{aligned}
\end{equation}
where $|t|$ is the number of different action traces that translate $S$ to $G$. In practice, we can throw the constant and evaluate the expectation using Monte Carlo estimation. We further adopt the breadth-first-search (BFS) node-ordering, a widely-used technique in sequential graph generation~\cite{you2018graphrnn, popova2019molecularrnn,shi*2020graphaf}, to reduce the number of valid transformation traces during sampling.
%We present the detailed sampling algorithm in Algorithm~\ref{alg:sampling}.
%The details of sampling procedure can be found in supplementary material.
%We present the details of \textcolor{red}{sampling procedure in  \ref{}}.
\iffalse
\begin{algorithm}[tb]
   \caption{Trace Sampling}
   \label{alg:sampling}
\textbf{Input}: $S$ synthon graph, $G$ reactant graph, $P$ maximum dependency distance in BFS, Adam hyperparameters $\beta_1, \beta_2$, use $\operatorname{Prod}(\cdot)$ as the product of elements across dimensions of a tensor


\begin{algorithmic}[1]
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}
\fi 

\subsubsection{Generation}\label{subsubsec:generation}

To generate a reactant graph, a natural way is to first sample a latent vector $z$ from the prior $p(z|S)$, then sample a trace of graph transformations from $p(t | z, S)$ (Section~\ref{subsubsec:generative_model}), and finally apply these transformations to the synthon $S$. However, in our proposed generative model, the probability of invalid actions will be non-zero even if the model is well-trained. As a result, any reactant molecules including invalid ones can be generated if sampling is arbitrarily long. Besides, this process also suffers from the non-trivial exposure bias problem~\cite{bengio2015scheduled}. To overcome the above obstacles 
% and incorporate chemical validity check
during sampling, we design a beam search sampling process as follows.

%figure if need????
Consider a beam search with size of $k$. 
For the graph generation in the $i^{th}$ step, we maintain a candidate set $\mathcal{S} = \{S^{i,j}\}_{j=1}^k$ with size $k$.
At the $i^{th}$ transformation step, we first calculate the probabilities of all possible actions and sort them, and then select the top $k$ ranked valid actions for each candidate graph $S^{i-1, j}$ in $\mathcal{S}$. Once this is done for $k$ graphs in $\mathcal{S}$, the top $k$ graphs among all the generated $k^2$ graphs are then selected as the candidates for the next $(i+1)^{th}$ transformation step. During this beam search, a translation branch will stop if $i$ reaches the predefined maximum transformation step or $a_i^1$ indicates a termination. In this scenario, the current graph will be added into a set $\mathcal{G}$, and the whole beam search terminates once all translation branches stop.
%the number of graphs in $\mathcal{G}$ reaches the predefined number.
%We finally choose top $k$ graphs in $\mathcal{G}$ ranked by their likelihood as the final predictions.
When the beam search finishes, the top $k$ graphs in $\mathcal{G}$,  ranked by their likelihoods, will be collected as the final predicted graphs.

\subsection{Scalability Analysis}
Both the Reaction Center Identification and the Variational Graph Translation modules in our \modelname framework bypass the deployment of reaction templates  and take advantage of the representation power of the molecular graph embeddings. As a result, the model size of \modelname scales linearly  \textit{w.r.t} the maximum number of atoms in the molecules and is invariant to the quantity of rules and reactions in the given data sets, making it highly scalable to larger data sets.









































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\subsubsection{Generation Process}
The generation process of a reactant $G$ is as follows: given a synthon $S$, we first sample a latent vector $z$ from a  prior distribution $z \sim P(z|S)$, and then $G$ is generated conditioned on
$z$ as well as $S$ via a series of graph transformation starting from $S$. Formally, the generation process can be characterized by the following probabilistic equation:
\begin{equation}\label{eq:vae_factorize}
P(G | S) = \sum\limits_z P(G |z, S) P(z | S)
\end{equation}
where $P(G | z, S)$ is parameterized by a novel graph decoder. 
%The optimization strategy follows a conditional variational autoencoder. 
We describe the details of variational graph translation module in the following paragraphs.
%Maximizing the log likelihood of the observed translation pair, i.e., $logP(G|S)$

\paragraph{Graph Encoder}

\paragraph{Graph Decoder}

\paragraph{Learning}
\fi


\iffalse
\subsection{Reactants Generation via Variational Graph Translation}
In this section, we elaborate the procedure that how synthons are translated into the final reactant graphs through our proposed variational graph translation module.
Given an chemical reaction $(\{G_i\}_{i=1}^{N_1}, G_p)$, we denote the set of synthons extracted from $G_p$ (Section~\ref{subsec:reaction_center}) as $\{S_i\}_{i=1}^{N_1}$. For simplicity, we omit the subscript and denote a translation pair $t$ as $(S, G)$. In this module we aim to learn a conditional generative model $p(G|S)$ that recover the reactant molecule domain ($G_i$) from the synthon molecule domain ($S_i$). In this scenario, a common problem is that the same synthon can be translated to different reactants which is known as the multi-modal problem.
% Note that $\mathcal{F}$ is a many-to-many mapping, i.e., a synthon can be translated to different reactants while a reactant can also be translated from different synthons. 
In order to mitigate this multi-modal problem and encourage the module to model the diverse distribution of reactants, we incorporate a low-dimensional latent vector $z$ to capture the uncertainty for the graph translation process.
%, and adopt an encoder-decoder architecture for the graph translation.


\subsubsection{The Generative Model}\label{subsubsec:generative_model}
We define the translation of a synthon $S$ to the final reactant $G$ as a conditional generative procedure, where $G$ is generated conditioned on the $S$ and a latent vector $z$. Precisely, we first autoregressively generate a sequence of graph transformation actions $\mathcal{T}_{1:T} = (a_1, \cdots, a_T)$, and then applying them on the initial synthon graph $S$. Here $a_t$ is a one-step graph transformation (action).
\textcolor{red}{add the reason that we choose to model this distribution instead of $p(G| z, S)$}.
We propose to model the distribution $p(\mathcal{T}_{1:T} | z, S)$ over the sequence of graph transformations. Once it is done, a synthon can be translated into a reactant by sampling action sequences from the distribution. Next, we describe the details of the generative procedure.

Assuming each action is only conditioned on the graph that have been modified so far, the joint distribution $p(\mathcal{T}_{1:T} | z, S)$ can be naturally factorized as follows:
\iffalse
\begin{equation}
p(\mathcal{T}_{1:T} | z, S) = p(a_{1} | z, S) \prod\limits_{i=2}^T p(a_{i} | z, S, \mathcal{T}_{1:i-1})
\end{equation}
\fi

\begin{equation}\label{eq:trace_fact}
p(\mathcal{T}_{1:T} | z, S) =
\prod\limits_{i=1}^T p(a_{i} | z, S^{i-1})
\end{equation}
where $S^{i}$ denote the graph after applying the sequence of actions $\mathcal{T}_{1:i}$ to $S$, and $S^0 = S$. 
Before we introduce the parameterization of distribution $P(a_{i} | z, S^{i-1})$, we formally introduce the definition of an action. An action $a_i$ is a tuple with four elements:
\begin{equation}
a_i = (a_{i}^1, a_{i}^2, a_{i}^3, a_{i}^4)
\end{equation}
Assuming the number of all different atoms is $m$, then $a_{i}^1 \in \{0, 1\}^2$ indicates the termination of graph transformations; $a_{i}^2 \in \{0, 1\}^n$ indicates the first node to focus; $a_{i}^3 \in \{0, 1\}^{n+m}$ indicates the second node to focus; $a_{i}^4 \in \{0, 1\}^b$ indicates the type of bond between two nodes. The distribution $p(a_{i} | z, S^{i-1})$ can then be factorized into three parts: (1) termination prediction $p(a_{i}^1 | z, S^{i-1})$; (2) nodes selection $p(a_{i}^{2:3}, | z, S^{i-1}, a_{i}^1) $; (3) edge labeling $p(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3})$.
We introduce the parameterization of these distributions in the following paragraphs.


\paragraph{Termination Prediction}
Denote a $L$-layer R-GCN (Section~\ref{subsec:rgcn}) that can compute the node embeddings of an input graph as $\mathcal{R}(\cdot)$.
We parameterize the distribution as:
\begin{equation}\label{eq:term_pred}
\begin{aligned}
&H = \mathcal{R}(S^{i-1}), \  h_{S}= \operatorname{Readout} (H)  \\
&p(a_{i}^1 | z, S^{i-1}) = 
\tau\big(m_t(h_{S}, z)\big)
\end{aligned}
\end{equation}
where $\tau(\cdot)$ denotes the softmax function, and $m_t(\cdot)$ is a feedforward networks. At each transformation step, we sample $a_{i}^1 \sim p(a_{i}^1 | z, S^{i-1})$. If $a_{i}^1$ indicates the termination, the graph translation stops, and current graph $S^{i-1}$ is treated as the final reactant generated by the module.
\paragraph{Nodes Selection}
Let the set of possible atoms to be added during graph translation be $\{v_1, \cdots, v_m\}$ and denote the collection as $V= \bigcup_{i=1}^m v_i$.
We first extend the graph $S^{i-1}$ to $\tilde{S}^{i-1} = S^{i-1} \bigcup V$.
The first node is selected from atoms in $S^{i-1}$, while the second node is selected from $\tilde{S}^{i-1}$ conditioned on the first node, by concatenating its embeddings with embeddings of each atom in $\tilde{S}^{i-1}$:
\begin{equation}\label{eq:node_select}
\begin{aligned}
&p(a_{i}^2 | z, S^{i-1}, a_{i}^1) = \tau
\big(
\beta^1 \odot
m_f(\mathcal{R}(\tilde{S}^{i-1}), z)
\big)\\
&a_{i}^2 \sim p(a_{i}^2 | z, S^{i-1}, a_{i}^1)\\
&p(a_{i}^3 | z, S^{i-1}, a_{i}^{1:2}) = \tau
\big(
\beta^2 \odot
m_s(\mathcal{R}(\tilde{S}^{i-1}), z, a_{i}^2)
\big)\\
&a_{i}^3 \sim p(a_{i}^3 | z, S^{i-1}, a_{i}^{1:2})\\
\end{aligned}
\end{equation}
where $m_f(\cdot)$ and $m_s(\cdot)$ are feedforward networks. $\beta^1$ and $\beta^2$ are masks to zero out the probability of certain atoms being selected.  $\beta^1$ forces the module to select node from $S^{i-1}$, and $\beta^2$ prevents the first node being selected again. 
It is important to note that only the second node can be selected from $V$, and it corresponds to adding a new atom to $S^{i-1}$.
The distribution of node selection $p(a_{i}^{2:3}, | z, S^{i-1}, a_{i}^1)$ is the product of two conditional distribution described above.
\paragraph{Edge Labeling}
The distribution for edge labeling is parameterized as follows:
\begin{equation}\label{eq:edge_label}
\begin{aligned}
&p(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3}) = \tau
\big(
m_e(\mathcal{R}(\tilde{S}^{i-1}), z, a_{i}^{2:3})
\big)\\
&a_{i}^4 \sim P(a_{i}^4 | z, S^{i-1}, a_{i}^{1:3})\\
\end{aligned}
\end{equation}
where $m_e(\cdot)$ is a feedforward networks. 

We leave all the details of feedforward networks described above as well as other architectures in \ref{}. Note that the knowledge about reaction classes can be incorporated to the input of each feedforward networks if available.

Given these distributions,
the joint distribution $p(\mathcal{T}_{1:T} | z, S)$ can be parameterized according to~\cref{eq:trace_fact,eq:term_pred,eq:node_select,eq:edge_label}. 
Finally, the probability of translating the synthon $S$ to the final reactant $G$ can be computed, by enumerating all possible graph transformation sequences that translate $S$ to $G$: 
\begin{equation}\label{eq:logp_gzs}
P(G|z, S) = \sum\limits_{\mathcal{T}}
P(\mathcal{T}_{1:T} | z, S)
\end{equation}

\subsubsection{Learning}
To learn the parameters of our variational graph translation module, we aim to maximize the log likelihood of the observed translation pair, \textit{i.e.}, $logP(G|S)$. Directly optimizing the objective involves marginalizing the latent variable $z$, which is computationally intractable. We turn to the standard amortized variational inference~\citep{kingma2014vae} by introducing an approximate posterior $q(z|G, S)$, which is modeled as a Gaussian distribution to allow effectively sampling $z$ via reparameterization trick.
%with a mean of $\mu$ and a variance of $\text{diag}(\sigma^2)$. 
The mean and log variance of $q(z|G, S)$ is parameterized as follows:
\begin{equation}
\begin{aligned}
& \mu = m_{\mu}(h_G \Vert h_S)\\
& \text{log}\sigma^2 = m_{\sigma}(h_G \Vert h_S)\\   
& q(z|G, S) = \mathcal{N}(z \vert \mu, \text{diag}(\sigma^2)) \\
\end{aligned}
\end{equation}
where $h_G, h_S$ are graph embeddings of $G, S$ computed by a R-GCN. $m_{\mu}(\cdot), m_{\sigma}(\cdot)$ are feedforward networks. The evidence lower bound (ELBO) is then defined as:
\begin{equation}
\mathcal{L}_{\text{ELBO}} = \mathbb{E}_{z \sim q}[\text{log}P(G|z,S)] - \operatorname{KL}[q(z|G, S) \Vert p(z|S)]
\end{equation}
where $\operatorname{KL}[q(\cdot) \Vert p(\cdot)]$ is the Kullback-Leibler divergence between $q(\cdot)$ and $p(\cdot)$. We further take a standard Gaussian prior $p(z|S) = \mathcal{N}(z | 0, I)$. 

\paragraph{Efficient Training}
The computation of $\text{log}P(G|z,S)$ (eq.~\ref{eq:logp_gzs}) is expensive as it
requires summation over all graph transformation sequences that translate $S$ to $G$. 
Here we introduce two strategies that perform well empirically. 
We first show that $\text{log}P(G|z,S)$ is lower bounded by the expected log likelihood of all the sequences that translate $S$ to $G$ using Jensen{'}s inequality:
\begin{equation}
\begin{aligned}
\text{log}P(G|z, S) &= \text{log}\sum\limits_{\mathcal{T}}
P(\mathcal{T}_{1:T} | z, S)\\
&\geq \text{log}Z + \frac{1}{Z}\sum\limits_{\mathcal{T}}\text{log}P(\mathcal{T}_{1:T} | z, S)
\end{aligned}
\end{equation}
where $Z$ is the number of different sequences that translate $S$ to $G$. In practice, we can throw the constant and evaluate the expectation using Monte Carlo estimation. We further adopt the breadth-first-search (BFS) node-ordering, a widely-used technique in sequential graph generation~\cite{you2018graphrnn, popova2019molecularrnn,shi*2020graphaf}, to reduce the number of valid transformation sequences during sampling. We present the details of sampling procedure in \ref{}.

\subsubsection{Generation}\label{subsubsec:generation}
To generate a reactant graph, a simple way is to first sample a latent $z$ from prior $p(z|S)$, then sample a sequences of graph transformations from $p(\mathcal{T}_{1:T} | z, S)$ (Section~\ref{subsubsec:generative_model}), and finally apply these transformations to the synthon $S$. However, the whole procedure is inefficient, and the reactant generated in this way may be invalid, as the probability of generating invalid molecules is non-zero even if the model is well-trained and any molecule can be generated if sampling is arbitrary long.
To accelerate the sampling procedure and incorporate chemical validity check during the generation, we introduce a way to efficiently generate valid reactants via beam search.

%figure if need????
Assume we use beam search with size $k$. 
We maintain a candidate set $\mathcal{S} = \{S^{i,j}\}_{j=1}^k$ with size $k$ for $i^{th}$ step during generation.
At  $i^{th}$ transformation step, we sample a set of actions for each candidate graph $S^{i-1, j}$ in $\mathcal{S}$, where top $k$ actions ranked by probability that transform $S^{i-1, j}$ into valid graphs are selected. Once this is done for $k$ graphs in $\mathcal{S}$, top $k$ graphs among all newly-generated $k^2$ graphs are selected as candidate for the next step. If translation of one branch stops, the current graph is added into a set $\mathcal{G}$. The whole beam search stops if $i$ reaches the max step or the number of graphs in $\mathcal{G}$ reaches the predefined number. We choose top $k$ graphs in $\mathcal{G}$ ranked by their log likelihood as the final predictions.
\fi




==> Retrosynthesis Camera Ready/4-experiment.tex <==
\section{Empirical Studies}
%Next, we move to evaluate the\ effectiveness of our proposed G2Gs framework.
%In this section, we first describe our experimental setups, and then discuss the quantitative results on retrosynthesis prediction. Finally, we detail an ablation study and visualize some prediction cases to help better understand our proposed model.  

%We also present some real cases including both the successful and failed ones on retrosynthesis prediction with our G2Gs framework. 
\subsection{Experiment Setup}
\textbf{Data }
%We evaluate our approach on the benchmark data set, USPTO-50k, which contains 50k atom-mapped reactions classified into 10 reaction types. Following~\citep{liu2017retro_seq2seq}, we randomly select 80\% of all reactions as training set and randomly split the rest into validation and test set of equal size. The statistics of the data set are show in Table~\ref{tab:data_info}.
We evaluate our approach on the widely used benchmark data set USPTO-50k, which contains 50k atom-mapped reactions with  10 reaction types. Following~\citep{liu2017retro_seq2seq}, we randomly select 80\% of the reactions as training set and divide the rest into validation and test sets with equal size. 
%The statistics of the data set are in Table~\ref{tab:data_info}.

\iffalse
\begin{table}[hb]
\centering

 \vspace{-7pt}
 \caption{Statistics of the evaluation data set.}  
 \vspace{1mm}
 %\resizebox{\columnwidth * 0.75}{!}{
 %\setlength{\tabcolsep}{8mm}{
 \begin{tabular}{ll}
  %\begin{tabular}{cc}
    	\toprule
    	\# train & 40,008 \\
    	\# val & 5,001 \\
    	\# test & 5,007 \\
    	\# reaction types & 10 \\
    	\# reactions with 0 reaction center & 14,122 \\
    	\# reactions with 1 reaction center & 34,819 \\
    	\# reactions with $\geq 2$ reaction centers & 1, 075 \\    	
    	\bottomrule
    \end{tabular}
    %}
	\vspace{-3pt}
\label{tab:data_info}  
\end{table}
\fi

\textbf{Baselines }
%write this part after related is done.
%We compare the proposed \modelname with the following baselines: the \textbf{seq2seq}~\citep{liu2017retro_seq2seq} is a template-free approach that learn a LSTM~\citep{lstm1997} to translate the SMILES strings of target molecules to those of reactant molecules; the \textbf{transformer}~\citep{pavel2019retro_transformer} is also based on neural sequence-to-sequence model implemented with Transformer~\citep{vaswani2017transformer}; the \textbf{retrosim}~\citep{Connor2017retrosim} is a data-driven method that selects template for target molecules based on similar reactions in the data set; the \textbf{neuralsym}~\citep{Marwin2017neuralsym} employs a neural model to rank templates; the \textbf{GLN}~\citep{Dai2019GLN} is a state-of-art method which samples templates and reactants jointly from the distribution learned by a conditional graphical model.
We evaluate our strategy using five comparison baselines,  including  two template-free and three template-based ones. In specific, \textbf{Seq2seq}~\citep{liu2017retro_seq2seq} is a template-free approach that learns a LSTM~\citep{lstm1997} to translate the SMILES strings of target molecules to reactants. \textbf{Transformer}~\citep{pavel2019retro_transformer} is also a neural sequence-to-sequence model, but it  leverages the learning power of the Transformer~\citep{vaswani2017transformer} for better sequential modeling. \textbf{Retrosim}~\citep{Connor2017retrosim} is a data-driven method that selects template for target molecules based on similar reactions in the data set. \textbf{Neuralsym}~\citep{Marwin2017neuralsym}  employs a neural model to rank templates for target molecules.  \textbf{GLN}~\citep{Dai2019GLN} is the state-of-the-art method, which samples templates and reactants jointly from the distribution learned by a conditional graphical model.

\iffalse
\begin{itemize}
    \item \textbf{seq2seq}~\citep{liu2017retro_seq2seq} is a template-free approach that learns a LSTM~\citep{lstm1997} to translate the SMILES strings of target molecules to reactants.
    \item   \textbf{transformer}~\citep{pavel2019retro_transformer} is also an approach based on neural sequence-to-sequence model, but leverages the power of the  Transformer~\citep{vaswani2017transformer}.
    \item  \textbf{retrosim}~\citep{Connor2017retrosim} is a data-driven method that selects template for target molecules based on similar reactions in the data set. 
    \item \textbf{neuralsym}~\citep{Marwin2017neuralsym} represents a method which employs a neural model to rank templates.
    \item \textbf{GLN}~\citep{Dai2019GLN} is the state-of-the-art method, which samples templates and reactants jointly from the distribution learned by a conditional graphical model.
\end{itemize}
\fi


\textbf{Evaluation Metrics }
Following the existing works~\cite{liu2017retro_seq2seq, Dai2019GLN}, we use the top-$k$ exact match accuracy as our evaluation metrics. For comparison purpose, we used $k$ with 1, 3, 5, and 10 in our experiments.  Also, the accuracy was computed by matching the canonical SMILES strings of the predicted molecules with the ground truth. 

\textbf{Implementation Details }
\modelname is implemented in Pytorch~\cite{pytorch2017automatic}. We use the open-source chemical software RDkit~\citep{RDKit} to preprocess molecules for the training and generate canonical SMILES strings for the evaluation. The R-GCN in \modelname is implemented with 4 layers and the embedding size is set as 512 for both modules.  We use latent codes of dimension $|z| = 10$.
We train our \modelname for 100 epochs with a batch size of 128 and a learning rate of 0.0001  with Adam~\citep{kingma2014adam} optimizer on a single GTX 1080Ti GPU card. The $\lambda$ is set as 20 for reaction center identification module, and the beam size is 10 during inference. %\textcolor{red}{value for 3.3.3?} 
The maximal number of transformation steps is set as 20.
We heuristically selected these values  based on the validation data set. 






\begin{table}[htbp]

\centering
 \vspace{-7pt}

 \caption{Top-$k$ exact match accuracy when reaction class is given. Results of all baselines are directly taken from~\citep{Dai2019GLN}.}  
 \vspace{1mm}
 %\resizebox{\columnwidth * 0.75}{!}{
 \setlength{\tabcolsep}{4mm}{
    \begin{tabular}{lcccc}
        \toprule
         \multirow{2}{*}{Methods}& \multicolumn{4}{c}{Top-$k$ accuracy \%} \\
        \cmidrule{2-5}
        & 1 & 3 & 5 & 10 \\
        \midrule
        \multicolumn{5}{c}{Template-free} \\
        \midrule
         Seq2seq & 37.4 & 52.4 & 57.0 & 61.7  \\
		 \modelname & {\bf 61.0} & {\bf 81.3} & {\bf 86.0} & {\bf 88.7}  \\
		 \midrule
		\multicolumn{5}{c}{Template-based} \\
		 \midrule
         %expertSys & 35.4 & 52.3 & 59.1 & 65.1 \\
		 Retrosim & 52.9 & 73.8 & 81.2 & 88.1 \\
		 Neuralsym & 55.3 & 76.0  & 81.4 & 85.1  \\
		 GLN & {\bf 64.2} & {\bf 79.1} & {\bf 85.2} & {\bf 90.0} \\
		 \bottomrule
    \end{tabular}
    }
	%\vspace{1mm}
    \vspace{-4pt}
    \label{tab:res_class}

\end{table}

\begin{table}[!h]
\centering
 \vspace{-7pt}
 \caption{Top-$k$ exact match accuracy when reaction class is unknown. Results of all baselines are taken from~\citep{Dai2019GLN}.}  
 \vspace{1mm}
 %\resizebox{\columnwidth * 0.75}{!}{
 \setlength{\tabcolsep}{4mm}{
    \begin{tabular}{lcccc}
        \toprule
         \multirow{2}{*}{Methods}& \multicolumn{4}{c}{Top-$k$ accuracy \%} \\
        \cmidrule{2-5}
         & 1 & 3 & 5 & 10 \\
        \midrule
        \multicolumn{5}{c}{Template-free} \\
        \midrule
         Transformer & 37.9 & 57.3 & 62.7 & /  \\
		 \modelname &  {\bf 48.9}&  {\bf 67.6} &  {\bf 72.5} & {\bf 75.5}  \\
		 \midrule
		\multicolumn{5}{c}{Template-based} \\
		 \midrule
		 Retrosim & 37.3 & 54.7 & 63.3 & 74.1 \\
		 Neuralsym & 44.4 & 65.3  & 72.4 & 78.9  \\
		 GLN & {\bf 52.5} & {\bf 69.0} & {\bf 75.6} & {\bf 83.7} \\
		 \bottomrule
    \end{tabular}
    }
	%\vspace{1mm}
	\vspace{-4pt}
	\label{tab:res_noclass}

\end{table}




%\subsection{Quantitative Results}
\subsection{Predictive Performance}\label{subsec:main_res}
%We evaluate the performance of the proposed \modelname in both reaction class known and reaction class unknown settings. Before we present the main results of the whole framework, we first report the performance of each module of our \modelname framwork.
We evaluate the top-$k$ exact match accuracy of the proposed approach in both reaction class known and reaction class unknown settings, with results  presented in  Tables~\ref{tab:res_class} and~\ref{tab:res_noclass}, respectively. 
The sets of reactant molecules are generated via beam search (Section~\ref{subsubsec:generation}) and ranked by their log likelihoods.  
%The results shown in Table~\ref{tab:res_class} and Table~\ref{tab:res_noclass} demonstrate that \modelname achieves competitive results on all four metrics in both settings. 

\begin{table}[htbp]
\centering
 \vspace{-5pt}
 \caption{Accuracy of the reaction center prediction module.}  
 \vspace{1mm}
 %\resizebox{\columnwidth * 0.75}{!}{
 %\setlength{\tabcolsep}{4mm}{
    \begin{tabular}{lcccc}
        \toprule
         \multirow{2}{*}{Setting}& \multicolumn{4}{c}{Top-$k$ accuracy \%} \\
        \cmidrule{2-5}
        & 1 & 2 & 3 & 5 \\
        \midrule
		 reaction class known &  90.2 &  94.5 &  94.9 &  95.0  \\
	     reaction class unknown &  75.8 &  83.9 &  85.3 &  85.6 \\

		 \bottomrule
    \end{tabular}
    %}
	\vspace{-4pt}
\label{tab:res_reaction_center}  

\end{table}
\begin{table}[htbp]
\centering
 \vspace{-7pt}
 \caption{Accuracy of the variational graph translation module.}  
 \vspace{1mm}
 %\resizebox{\columnwidth * 0.75}{!}{
 %\setlength{\tabcolsep}{4mm}{
    \begin{tabular}{lcccc}
        \toprule
         \multirow{2}{*}{Setting}& \multicolumn{4}{c}{Top-$k$ accuracy \%} \\
        \cmidrule{2-5}
        & 1 & 3 & 5 & 10 \\
        \midrule
		 reaction class known &  66.8 & 87.2 & 91.5 & 93.9  \\
	     reaction class unknown & 61.1  & 81.5  & 86.7  &  90.0  \\

		 \bottomrule
    \end{tabular}
    %}
	\vspace{-5pt}
\label{tab:res_vg2g}  

\end{table}

When compared with template-free approaches, results shown in Tables~\ref{tab:res_class} and~\ref{tab:res_noclass} demonstrate that the \modelname achieves competitive results on all the cases with different $k$. %namely with known and unknown reaction classes. 
In particular, our \modelname always outperforms the template-free baselines by a large margin, with up to 63\% relative improvement in terms of the top-1 exact match accuracy when the reaction class is known (the second column in Table~\ref{tab:res_class}), and up to 29\% relative improvement when the reaction class is unknown (the second column in Table~\ref{tab:res_noclass}). 

When consider the comparison with template-based baselines, the results in Tables~\ref{tab:res_class} and~\ref{tab:res_noclass} indicate that our \modelname approaches or outperforms the state-of-the-art method GLN~\citep{Dai2019GLN}, especially when the $k$ is small. %, making it particularly appealing in practice.
%\textcolor{red}{Intuitively, a small $k$ represents the challenging situation where....indicates that our method making it particularly appealing in practice. }
For example, when reaction class is given as a prior, our \modelname outperforms the GLN in terms of the top-3 and top-5 exact match accuracy.
%, with a relative improvement of 2.8
%\textcolor{red}{with \% and \%, respectively.}


\begin{figure*}[hbtp]
	\centering
    \includegraphics[width=.89\linewidth]{figure/latent.pdf}
     \vspace{-3pt}
    \caption{Visualization of the top-1 translation results (right four molecules) of a given product molecule (leftmost), which are conditioned on different latent vectors sampled from prior $\mathcal{N}(z | 0, I)$. The correct prediction provided is highlighted in red dashed box.}
    %\caption{Translation examples of our proposed framework. Given a specified product molecule (leftmost), the variational graph translation module enables us to generate diverse and valid reactant predictions (right). Among them, one is the same as the ground truth provided in training set (highlight the in red dashes), while the other three also obey the chemical rules.}
    % Illustration of the proposed variational graph translation module, including the encoder $q(z|G,S)$ (left) and the generative model $p(G|z,S)$ (right). The phases of the generation procedure is shown in the generative model. With a sampled latent vector $z$, the synthon graph $S$ enters a loop with nodes selection and edge labeling until the termination state is predicted.}
    \label{fig:latent}
\end{figure*}



\subsection{Ablation Study}
To  gain  insights into the working behaviours of  G2Gs, we conduct ablation studies in this section. %We first quantitatively  examine the power of the  two  modules in   G2Gs, and then show the  working behaviours of our method  through visualization. 

\begin{figure*}[ht]
\centering

\noindent\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=0.9\linewidth]{figure/right+template_v4-crop.pdf}
\vspace{-2pt}
\caption{Visualization of several successful cases. Templates for these reactions are summarized at the bottom of the figure.}
\label{fig:right_case_template}
\vspace{-5pt}
\end{minipage}%
\hfill
\noindent\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=0.9\linewidth]{figure/wrong_case_v3-crop.pdf}
\vspace{-2pt}
\caption{
Visualization of a mismatched case. Outcomes  of the reactions below the middle line are predicted by the forward reaction prediction model from~\citep{jin2017weisfeiler}.
}
\label{fig:wrong_case}
\vspace{-5pt}

\end{minipage}%


\centering
%\caption{Visualization of several successful cases and a failed case.}
\end{figure*}


\textbf{Effectiveness of the Reaction Center Identification Module }
%\textcolor{blue}{
We evaluate the top-$k$ accuracy of the reaction center identification module by comparing the true reaction center against the top-$k$ atom pairs with the highest reactivity scores above a threshold. 
The results in Table~\ref{tab:res_reaction_center} indicate that when the reaction class is given as a prior, \modelname can  precisely pinpoint the reaction center in most cases even for $k=1$. When the reaction class is unknown, the performance is slightly worse than the previous case, as a target molecule can usually be synthesized in different routes depending on what reaction type a chemist chooses, and thus the model tends to make predictions with low certainty. 
%The problem can be partially addressed by incorporating more information about reactions into the module, \textit{e.g.}, reagent and temperature. To strike a balance between performance and inference time, we choose $k=2$ for reaction center identification module in the subsequent experiments.
%} 

%These results indicates that the Reaction Center Identification module is able to accurately identify the centers in the given molecules to benefit the following module, namely the Variational Graph Translation component. 





\textbf{Impact of the Variational Graph Translation Module } 
To examine the  graph translation module, we first split synthons from products based on the true reaction centers (\textit{i.e.}, label matrix $Y$ in Section~\ref{subsec:reaction_center}), and then use the same strategy as in Section~\ref{subsec:main_res} to compute the top-$k$ exact match accuracies. As shown in Table~\ref{tab:res_vg2g}, the graph translation module achieves high accuracy on translating the given synthon graphs to reactant graphs, which is an important attribute to  the  superior performance of the proposed G2Gs framework. 
%By comparing Table~\ref{tab:res_class},~\ref{tab:res_noclass} and~\ref{tab:res_vg2g}, we








\iffalse
\begin{figure}[!h]
	\centering
    \includegraphics[width=.99\linewidth]{figure/right_v2-crop.pdf}
    \caption{Visualization of a successful case. The top-3 predictions are shown in the figure.}
    \label{fig:right_case}
\end{figure}
\fi

\textbf{Diverse Reactant Graph Generation} 
To observe the benefits brought by the latent vector used in  \modelname, Figure~\ref{fig:latent}  visualizes the top-1 translation results for a given  product molecule, which is randomly selected from the test set. In the figure, the right four molecules are generated, based on the same synthon (leftmost molecule in the figure), through randomly sampling from the prior distribution of the formed latent vector. 
Results in this figure suggest that, through sampling the latent vector formed, our method can generate diverse molecule structures. That is, sampling the learned latent vector,  an intrinsic process in  \modelname, powers our model to create diverse and valid reactant graphs, which represents an  appealing feature  for retrosynthesis prediction.  






\subsection{Case Study via Visualization}
%In this section,  we  visualize several randomly selected reactant graphs generated by our method, including cases that match the ground truth and ones missing the targets. 

In Figure~\ref{fig:right_case_template}, we show  cases where \modelname successfully identifies the reaction centers and translates the product graph to a set of reactant graphs that match the ground truth. %The reactant graphs shown in Figure~\ref{fig:latent} are top-1 translation results based on the same synthon (leftmost molecule in the figure) with different latent vectors, which demonstrate the capability of our \modelname to generate diverse and valid reactant graphs.
%As shown in Figure~\ref{fig:right_case_template}, our model makes the correct prediction with high certainty (top-1), and the top-3 prediction also shares similar graph structures with the ground truth, which may also be a valid synthesis route.
The synthesis routes shown in Figure~\ref{fig:right_case_template} can be divided into two groups, each of which corresponds to a reaction template presented at the bottom of the figure. These figures suggest that our model does learn domain knowledge from the data set. Such property of our method makes it 
an appealing solution to practical problems with limited  template knowledge. 


In Figure~\ref{fig:wrong_case}, we also present a case where none of the predictions matches the ground truth.
However, we note that this does not necessarily mean that our model fails to predict a synthesis route for the target molecule. This is because a molecule can be synthesized in multiple ways and the ground truth in the data set is not the only answer. To verify  this hypothesis, we employ a forward reaction prediction model~\citep{jin2017weisfeiler} to predict the product molecules based on the reactants generated by our model. As shown at the bottom of Figure~\ref{fig:wrong_case}, the predicted product exactly matches the target molecule of the retrosynthesis problem. This confirms that  the predictions made by \modelname are indeed potentially valid.






\iffalse

\begin{figure}[h]
	\centering
    \includegraphics[width=.99\linewidth]{figure/wrong_v0-crop.pdf}
    \caption{Visualization of a mismatched case. Outcomes of the reactions below the middle line are predicted by the forward reaction prediction model from~\citep{jin2017weisfeiler}.}
    \label{fig:wrong_case}
\end{figure}
\fi





==> Retrosynthesis Camera Ready/5-conclusion.tex <==
%\section{Conclusion}
\section{Conclusion and Outlook}

We novelly formulated retrosynthesis prediction as a graph-to-graphs translation task and proposed a template-free approach to attain the  prediction goal. In addition, 
 we devised a variational graph translation module to capture the uncertainty and to encourage diversity in the graph translation  process.  
 We also empirically verified the superior performance of our proposed method; our strategy outperformed the state-of-the-art  template-free counterpart by up to 63\% and  approached  the  performance obtained by the state-of-the-art template-based strategy, in terms of top-1 accuracy.
 Our method  excludes  domain knowledge and scales well to large datasets, making it  particularly attractive in practice.

 Our future work will include  extending our \modelname approach to embrace an end-to-end training paradigm and leveraging it to cope with  multi-step retrosynthesis tasks~\citep{corey1991logic}. 

\iffalse
In this paper we presented a novel graph-to-graphs framework called \modelname for retrosynthesis prediction. \modelname is a template-free approach composed of two modules: a reaction center identification module and a synthon-to-reactant variational graph translation module.
%\modelname is able to generate 100\% chemically valid prediction but does not require domain knowledge and scales well to large data sets.
Experimental results demonstrate that our method significantly outperforms the template-free baselines and achieves the comparable performance against the state-of-the-art template-based approaches, but excludes the need for domain knowledge and is much more scalable.
For future work, we plan to extend our \modelname to the challenging multi-step retrosynthesis~\citep{} analysis and also train the model with supervisions from both directions (\textit{i.e.}, reactants to products and products to reactants) to further improve the performance. further improve the performance.
\fi


